Heat content asymptotics for sub-Riemannian manifolds

We study the small-time asymptotics of the heat content of smooth non-characteristic domains of a general rank-varying sub-Riemannian structure, equipped with an arbitrary smooth measure. By adapting to the sub-Riemannian case a technique due to Savo, we establish the existence of the full asymptotic series: \begin{equation} Q_\Omega(t) = \sum_{k=0}^{\infty} a_k t^{k/2}, \qquad \text{as } t\to 0. \end{equation} We compute explicitly the coefficients up to order $k=5$, in terms of sub-Riemannian invariants of the domain and its boundary. Furthermore, we prove that every coefficient can be obtained as the limit of the corresponding one for a suitable Riemannian extension. As a particular case we recover, using non-probabilistic techniques, the order $2$ formula due to Tyson and Wang in the first Heisenberg group [J. Tyson, J. Wang, Comm. PDE, 2018]. An intriguing byproduct of our fifth-order analysis is the evidence for new phenomena in presence of characteristic points. In particular, we prove that the higher order coefficients in the expansion can blow-up in their presence. A key tool for this last result is an exact formula for the sub-Riemannian distance from a specific surface with an isolated characteristic point in the first Heisenberg group, which is of independent interest.

==> asymptotic.tex <==
\section{Heat content asymptotic}
In this section, we present a technique to compute the full asymptotic expansion of the \sr heat content, associated with the Dirichlet problem \eqref{eqn:dir_prob}, provided that the boundary of $\Omega$ has no characteristic points. To our knowledge, this technique first appeared in a work by A. Savo (see \cite{Savo-heat-cont-asymp}), for the Riemannian case, and it relies on a Riemannian mean value Lemma, a $1$-dimensional version of the Duhamel's principle and the recursive construction of a suitable algebra of operators involving the Riemannian Laplacian and the Riemannian normal derivative. Once a \sr mean value Lemma is available, the technique can be adapted without any substantial change to the \sr case, provided that the distance from $\partial\Omega$ is smooth, up to the boundary.

Notice that the \sr mean value Lemma allows a remarkable dimensionality reduction for our problem, indeed we can now relate the asymptotic expansion of the heat content, which, a priori, does not verify any known differential relation, with the asymptotic expansion of the function 
\begin{equation}
F(t,r)\coloneqq\int_{\om{r}}u(t,x)\dvol(x),
\end{equation}
which satisfies the non-homogeneous one-dimensional heat equation \eqref{eqn:nonhom_heat}.

\medskip

As the \sr principle of not feeling the boundary suggests, all the relevant information involved in the asymptotic expansion for the heat content, are concentrated near the boundary. Therefore, we would like to reduce our problem to a localized version of the heat content. 

\begin{defn}
\label{def:op_ILambda}
Let $M$ be a \sr manifold with volume $\omega$ and $\Omega\subset M$ be a connected and relatively compact subset of $M$. Let $\delta\colon\bar\Omega\to[0,\infty)$ be the distance function from $\partial\Omega$. Let us denote $\neighbd\coloneqq\{x\in\bar{\Omega};\ \delta(x)<\smallpar\}$. We define the operators $I$ and $\Lambda$, acting on the space $C_c^\infty(\neighbd)$, as
\begin{equation}
%\label{eqn:op_ILambda}
\begin{split}
I\phi(t,r) &= \int_{\om{r}}{(1-u(t,x))\phi(x)\omega_x},\\
\Lambda\phi(t,r) &= \int_{\bdom{r}}{(1-u(t,x))\phi(x)\omega_x},
\end{split}
\end{equation} 
for any $\phi\in C_c^\infty(\neighbd)$. Here $u(t,x)$ denotes the solution to \eqref{eqn:dir_prob}.
\end{defn}

Assuming that the boundary of $\Omega$, $\partial\Omega$, is a smooth hypersurface with no characteristic points implies that both $I\phi$ and $\Lambda\phi$ are smooth functions in $(0,\infty)\times[0,\infty)$ compactly supported in the $r$-variable, indeed for $r>\varepsilon$, the function $\phi$ vanishes. This property formalizes the idea, previously stated, of localizing the problem of finding the heat content asymptotic near $\partial\Omega$, indeed, we will look for an asymptotic expansion of $I\phi(t,0)$.

\subsection{First order asymptotic expansion for \texorpdfstring{$I\phi$}{Iphi}}
In this section, we develop a first order asymptotic expansion for $I\phi(t,0)$, as $t\to 0$. This comes directly from a single application of the Duhamel's principle. Recall the general $1$-dimensional Duhamel's principle: set $L\coloneqq \partial_t-\partial_r^2$, then, given any functions $w,v\in C^\infty((0,\infty)\times[0,\infty))$, for $[\alpha,\beta]\in(0,t)$, we have: 
%\begin{equation}
%\label{1D_duhamel_prin}
%\begin{split}
%&\int_0^\infty{(w(t-\alpha,r)v(\alpha,r)-w(t-\beta,r)v(\beta,r))dr}\\
			 %&= \int_\alpha^\beta{\int_0^\infty{( Lw(t-\tau,r)\cdot v(\tau,r)-w(t-\tau,r)\cdot Lv(\tau,r))dr}\ \negthinspace d\tau}\\
			 %&\ \ -\int_\alpha^\beta{\Big(w(t-\tau,r)\partial_rv(\tau,r)-v(\tau,r)\partial_rw(t-\tau,r)\Big)\bigg|_{r=0}^{r=\infty}d\tau},
%\end{split}
%\end{equation}
\begin{multline}
\label{eqn:1D_duhamel}
\int_0^\infty{(w(t-\alpha,r)v(\alpha,r)-w(t-\beta,r)v(\beta,r))dr}\\
			 = \int_\alpha^\beta{\int_0^\infty{( Lw(t-\tau,r)\cdot v(\tau,r)-w(t-\tau,r)\cdot Lv(\tau,r))dr}\ \negthinspace d\tau}\\
			 -\int_\alpha^\beta{\Big(w(t-\tau,r)\partial_rv(\tau,r)-v(\tau,r)\partial_rw(t-\tau,r)\Big)\bigg|_{r=0}^{r=\infty}d\tau},
\end{multline}
provided that the last integral exists finite.

Let us apply \eqref{eqn:1D_duhamel} with $v(t,r)\coloneqq F(t,r)$ where $F$ is just a smooth function such that, for each $t$ fixed, it is compactly supported in $[0,\infty)$ w.r.t. $r$, and $w(t,r)\coloneqq e(t,r,s)$, where $s\geq 0$ is fixed and $e$ is the heat kernel associated with the $1$D problem

\begin{equation}
\label{eqn:1D_neumann}
\left\{\begin{array}{llll}
Lu(t,r)&=&0,& \text{for }t>0,\ r\in(0,\infty) \\
u(0,r)&=&1,&\text{for }r\in(0,\infty)\\
\partial_ru(t,0)&=&0,& \text{for }t>0.
\end{array}\right.
\end{equation}
The problem \eqref{eqn:1D_neumann} is just the heat equation on the half-line with Neumann boundary condition, thus its kernel can be easily computed by reflection and is given by
\begin{equation}
e(t,r,s)\coloneqq \frac{1}{\sqrt{4\pi t}}\left(e^{-(r-s)^2/4t}+e^{-(r+s)^2/4t}\right) \ \ \text{for}\ t\in(0,\infty), \ r,s\in[0,\infty).
\end{equation}
Hence, since both $F$ and $e$ vanish as $r\to\infty$ and $e$ satisfies the Neumann boundary condition, \eqref{eqn:1D_duhamel} rewrites as
\begin{multline}
\int_0^\infty{(e(t-\alpha,r,s)F(\alpha,r)-e(t-\beta,r,s)F(\beta,r))dr}\\= -\int_\alpha^\beta{\int_0^\infty{e(t-\tau,r,s)LF(\tau,r)dr}\ \negthinspace d\tau}+\int_\alpha^\beta{e(t-\tau,0,s)\partial_rF(\tau,0)d\tau},
\end{multline}
for any $[\alpha,\beta]\subset (0,t)$ and $s\geq 0$. Thus, for $\alpha\to 0$ and $\beta\to t$, we finally obtain:
\begin{multline}
\label{eqn:1D_duhamel2}
\int_0^\infty{e(t,r,s)F(0,r)dr}-F(t,s) \\= -\int_0^t{\int_0^\infty{e(t-\tau,r,s)LF(\tau,r)dr}\ \negthinspace d\tau}+\int_0^t{e(t-\tau,0,s)\partial_rF(\tau,0)d\tau},
\end{multline}
whenever the quantities $F(0,r)$, $LF(\tau,r)$, $\partial_rF(\tau,0)$ are well-defined and the integrals are finite. We will need a technical Lemma, whose proof is included in the more general statement of Lemma \ref{lem:iter_L}, which can be found in the Appendix \ref{app:B}.

\begin{lem}
\label{lem:op_LI}
Let $M$ be a \sr manifold with volume $\omega$ and $\Omega\subset M$ be a connected and relatively compact subset of $M$, whose boundary is a smooth hypersurface with no characteristic points. Denote by $\delta\colon\bar\Omega\to[0,\infty)$ be the distance function from $\partial\Omega$ and by $\neighbd\coloneqq\{x\in\bar{\Omega};\ \delta(x)<\smallpar\}$. Then, as an operator on $C_c^\infty(\neighbd)$:
\begin{equation}
%\label{eqn:op_LI}
LI=\Lambda\normal+I\deltasr,
\end{equation} 
where $\normal$ is the operator defined by:
\begin{equation}
\label{eqn:sr_normal}
\normal\phi\coloneqq 2g\left(\grad\phi,\grad\delta\right)+\phi\deltasr\delta,\qquad\forall\,\phi\in C_c^\infty(\neighbd).
\end{equation}
\end{lem}\todo{Non si capisce perché sia stato fatto il \sr mean value Lemma. Forse sarebbe meglio inserire la dimostrazione qui?}

\begin{thm}
\label{thm:1ord_Iphi}
Under the same hypotheses of Lemma \ref{lem:op_LI}, let $\phi\in C_c^\infty(\neighbd)$. Then, the function $I\phi(t,0)$ has the following expansion:
\begin{equation}
\label{eqn:1ord_Iphi}
I\phi(t,0)=\frac{2}{\pi}\int_{\partial\Omega}{\phi(y) \area}\sqrt{t}+O(t),\quad\text{as }t\to 0.
\end{equation}
\end{thm}

\begin{proof}
The statement follows directly from \eqref{eqn:1D_duhamel2}, with $F(t,r)=I\phi(t,r)$. We should only check that the quantities $I\phi(0,r)$, $LI\phi(\tau,r)$ and $\partial_rI\phi(\tau,0)$ makes sense. The first one is given by $I\phi(0,r)=0$, being the initial datum $u(0,x)=1$ on $\Omega$, while $\partial_rI\phi(t,0)=-\Lambda\phi(t,0)=-\int_{\partial\Omega}{\phi}$ due to the boundary condition. On the other hand, the quantity $LI\phi(t,r)$ is well-defined as $t\to 0$, for any $r\geq 0$, indeed, from Lemma \ref{lem:op_LI}, $LI=\Lambda \normal+I\deltasr$, and the functions $\normal\phi,\deltasr\phi\in C_c^\infty(\neighbd)$. Therefore, applying \eqref{eqn:1D_duhamel2}, we obtain:
\begin{multline}
I\phi(t,0)=\int_0^\infty{e(t,r,0)I\phi(0,r)dr}-\frac{1}{\sqrt{\pi}}\int_0^t{\partial_rI\phi(\tau,0)(t-\tau)^{-1/2}d\tau}\\+\int_0^t{\int_0^\infty{e(t-\tau,r,0)LI\phi(\tau,r)dr}\ \negthinspace d\tau}.
\end{multline}
Thus, substituting the expressions with their values,
\begin{equation}
I\phi(t,0)=\frac{1}{\sqrt{\pi}}\int_{\partial\Omega}{\phi \area}\int_0^t{(t-\tau)^{-1/2}d\tau}+\int_0^t{\int_0^\infty{e(t-\tau,r,0)LI\phi(\tau,r)dr}\ \negthinspace d\tau}.
\end{equation}
Since $\int_0^t{(t-\tau)^{-1/2}d\tau}=2\sqrt{t}$, it's enough to prove that the remainder is an $O(t)$ to conclude the proof. Notice that 
\begin{equation}
\left|LI\phi(t,r)\right|=\left|\Lambda \normal\phi(t,r)+I\deltasr\phi(t,r)\right|\leq C_1\|\normal\phi\|_{L^\infty(\Omega)}+C_2\|\deltasr\phi\|_{L^\infty(\Omega)}\eqqcolon C,
\end{equation} 
having used the maximum principle to conclude that $|1-u(t,x)|\leq 1$. Thus, we obtain
\begin{align}
\left|\int_0^t{\int_0^\infty{e(t-\tau,r,0)LI\phi(\tau,r)dr}\ \negthinspace d\tau}\right| &\leq C\int_0^t{\int_0^\infty{e(t-\tau,r,0)dr}\ \negthinspace d\tau}\\
																																												 &= C\int_0^t{\frac{1}{\sqrt{\pi (t-\tau)}}\int_0^\infty{e^{-r^2/4(t-\tau)}dr}\ \negthinspace d\tau}\\
																																												 &= Ct,
\end{align}
implying statement \eqref{eqn:1ord_Iphi}.
\end{proof}

\subsection{Full asymptotic expansion for \texorpdfstring{$I\phi$}{Iphi}}
We would like to iterate the Duhamel's principle to obtain higher order asymptotic expansion of $I\phi(t,0)$, indeed Theorem \ref{thm:1ord_Iphi}suggests that, for any $m\in\N$, a sufficiently high number of iterations of formula \eqref{eqn:1D_duhamel} should provide an explicit expression for the remainder of order $m$, and then an asymptotic expansion. Unfortunately, while for the first order expansion the Duhamel's principle can be applied directly to the function $I\phi$, for the iterations $m\geq 1$, this is no longer true. Indeed, already the first iteration of \eqref{eqn:1D_duhamel} involves a term of the form
$\partial_tI(t,r)$, which is given by:
\begin{equation}
\partial_tI\phi(t,r)=-\int_{\om{r}}{\partial_tu(t,x)\phi(x)\omega_x}.
\end{equation}
The behavior of this term is not clear when $r=0$ and $t$ approaches $0$, since $u(t,x)$ is not smooth up to $t=0$, when $x\in\partial\Omega$. In particular, $\partial_tu(t,x)$ may not be integrable on $\Omega$ as $t\to 0$. To avoid this technical issue, we introduce an approximation of the operators $I$ and $\Lambda$, for which we will be able to apply iterations of the Duhamel's principle for any $m\geq 1$. We refer to Appendix \ref{app:B}, for further details. 

%\begin{thm}
%\label{thm:2nd_order_exp_I_phi}
%Let $\phi\in C_c^\infty(\neighbd)$. Then, the function $I\phi(t,0)$ has the following expansion
%\begin{equation}
%\label{2nd_order_exp_I_phi}
%I\phi(t,0)=\frac{2}{\sqrt{\pi}}\int_{\partial\Omega}{\phi \area}\sqrt{t}+\frac{1}{2}\int_{\partial\Omega}{\normal\phi \area}t+O(t^{3/2}),\quad\text{as }t\to 0.
%\end{equation}
%\end{thm}
%
%\begin{proof}
%Let us divide the proof in steps.
%
%\textit{Step 1}: Apply the iterated Duhamel's principle for $m=2$, with $F(t,r)=I_\epsilon\phi(t,r)$, $\epsilon\in(0,\varepsilon)$ and perform the limit as $\epsilon\to 0$. 
%
%\noindent Firstly, writing formula \eqref{eqn:iter_duhamel} for $I_\epsilon\phi$, we obtain
%\begin{multline}
%I_\epsilon\phi(t,0)=\sum_{k=0}^2{\frac{t^k}{k!}\int_0^\infty{e(t,r,0)L^kI_\epsilon\phi(0,r)dr}}+\frac{1}{\sqrt{\pi}}\sum_{k=0}^2{\frac{1}{k!}\int_0^t{L^k\Lambda_\epsilon\phi(\tau,0)(t-\tau)^{k-1/2}d\tau}}\\+\frac{1}{2}\int_0^t{\int_0^\infty{e(t-\tau,r,0)L^{3}I_\epsilon\phi(\tau,r)(t-\tau)^2dr}\ \negthinspace d\tau}.
%\end{multline}
%Secondly, performing the limit of $I_\epsilon\phi$ for $\epsilon\to 0$, we get, from the dominated convergence Theorem, 
%\begin{equation}
%I_\epsilon\phi(t,r)\xrightarrow{\epsilon\to 0}I\phi(t,r),
%\end{equation}
%hence, we see that
%\begin{multline}
%\label{lim_I_eps_after_duh}
%I\phi(t,0)=\sum_{k=0}^2\lim_{\epsilon\to 0}\Bigg(\frac{t^k}{k!}\int_0^\infty{e(t,r,0)L^kI_\epsilon\phi(0,r)dr}\\+\frac{1}{\sqrt{\pi}k!}\int_0^t{L^k\Lambda_\epsilon\phi(\tau,0)(t-\tau)^{k-1/2}d\tau}\Bigg)+O(t^{3/2}),
%%\frac{1}{2}\int_0^t{\int_0^\infty{e(t-\tau,r,0)L^{3}I_\epsilon\phi(\tau,r)(t-\tau)^2dr}\ \negthinspace d\tau}.
%\end{multline}
%where, accordingly to Lemma \ref{lem:uniform_est_reminder}, the reminder has been neglected since we are looking for an asymptotic expansion of order $t^{3/2}$. Notice that the estimate of the reminder is uniform with respect to $\epsilon$.
%
%\textit{Step 2}: Compute $\lim_{\epsilon\to 0}\int_0^\infty{e(t,r,0)L^kI_\epsilon\phi(0,r)dr}$ for $k=0,1,2$.
%\begin{mydescription}
%\item[$(k=0)$] Using the explicit expression provided by Lemma \ref{lem:hp_idp_aux}, we can write
%\begin{equation}
%\int_0^\infty{e(t,r,0)I_\epsilon\phi(0,r)dr}=\int_{\omprime{\epsilon}}{\phi(x)\left(\smallerint{0}{\delta(x)}{e(t,r,0)dr}\right) \dvol(x)}\xrightarrow{\epsilon\to 0}0,
%\end{equation}
%by the dominated convergence Theorem, since the integrand $\left|\phi(x)\left(\smallerint{0}{\delta(x)}{e(t,r,0)dr}\right)\right|\leq |\phi(x)|$, and $\omprime{\epsilon}\searrow \emptyset$.
%%by the dominated convergence Theorem, since the integrand 
%%\begin{equation}
%%\left|\phi(x)\left(\smallerint{0}{\delta(x)}{e(t,r,0)dr}\right)\right|\leq |\phi(x)|,
%%\end{equation}
%%and $\omprime{\epsilon}\searrow \emptyset$.
%\item[$(k=1)$] We rely on Lemma \ref{lem:iter_L} to compute $LI_\epsilon=\Lambda_\epsilon \normal+I_\epsilon\deltasr$. As in the previous case, the term involving $I_\epsilon$ is an $o(\epsilon)$, therefore we should only compute $\lim_{\epsilon\to 0}\int_0^\infty{e(t,r,0)\Lambda_\epsilon \normal\phi(0,r)dr}$, which can be done using again Lemma \ref{lem:hp_idp_aux}:
%\begin{equation}
%\int_0^\infty{e(t,r,0)\Lambda_\epsilon \normal\phi(0,r)dr}=\int_{\omprime{\epsilon}}{\normal\phi(x)e(t,\delta(x),0)\dvol(x)}\xrightarrow{\epsilon\to 0}0,
%\end{equation}
%by dominated convergence Theorem.
%\item[$(k=2)$] Finally, proceeding as in the case $k=1$, we get that the only term that may give a contribution is 
%\begin{equation}
%\int_0^\infty{e(t,r,0)\partial_tI_\epsilon \normal^2\phi(0,r)dr}=-\int_{\om{\epsilon}}{\deltasr\Big(\normal^2\phi\smallerint{0}{\delta(x)}{e(t,r,0)dr}\Big)(x) \dvol(x)}.
%\end{equation}
%The integrand function is of the form $\deltasr(\varphi(\psi\circ\delta))$, hence may be discussed as follows
%\begin{align}
%\int_{\om{\epsilon}}\deltasr(\varphi(\psi\circ\delta))\dvol &= \int_{\om{\epsilon}}\deltasr(\varphi(\psi\circ\delta)) \dvol\\
																														 %&= \int_{\om{\epsilon}}\left((\psi\circ\delta)\deltasr \varphi+(\psi'\circ\delta)\normal\varphi+(\psi''\circ\delta)\varphi\right) \dvol\\
																														 %&= \psi(\epsilon)\int_{\om{\epsilon}}\deltasr \varphi \dvol+\psi'(\epsilon)\int_{\om{\epsilon}}\normal\varphi \dvol+\psi''(\epsilon)\int_{\om{\epsilon}}\varphi \dvol\\
																														 %&\xrightarrow{\epsilon\to 0}\psi(0)\int_{\Omega}\deltasr \varphi \dvol+\psi'(0)\int_{\Omega}\normal\varphi \dvol+\psi''(0)\int_{\Omega}\varphi \dvol.
%\end{align}
%In our case $\varphi(x)=N^2\phi(x)$ and $\psi(r)=\int_0^re(t,s,0)ds$, implying $\psi(0)=0$, $\psi'(0)=\frac{1}{\sqrt{t\pi}}$, $\psi''(0)=0$, thus
%\begin{equation}
%\int_0^\infty{e(t,r,0)\partial_tI_\epsilon \normal^2\phi(0,r)dr}\xrightarrow{\epsilon\to 0}-\frac{1}{\sqrt{t\pi}}\int_{\Omega}\normal^3\phi \dvol.
%\end{equation}
%\end{mydescription}
%\hspace{\parindent}\textit{Step 3}: Compute $\lim_{\epsilon\to 0}\int_0^t{L^k\Lambda_\epsilon\phi(\tau,0)(t-\tau)^{k-1/2}d\tau}$ for $k=0,1,2$.
%\begin{mydescription}
%\item[$(k=0)$] As in the previous step, we use Lemma \ref{lem:hp_idp_aux} to characterize $\Lambda_\epsilon(\tau,0)$, obtaining
%\begin{equation}
%\int_0^t{\Lambda_\epsilon\phi(\tau,0)(t-\tau)^{-1/2}d\tau}=2\int_{\partial\Omega}{\phi(x)\dvol(x)}\sqrt{t},
%\end{equation}
%which clearly doesn't change in the limit for $\epsilon\to 0$.
%\item[$(k=1)$] Recall the expression for $L\Lambda_\epsilon=\Lambda_\epsilon\left(-\normal^2+\deltasr\right)-I_\epsilon\deltasr \normal+\partial_tI_\epsilon \normal$, namely we have three different terms. The first one, of the form $\Lambda_\epsilon\varphi$, can be discussed as in the previous case, therefore is negligible, being an $O(t^{3/2})$. The second one is given by
%\begin{equation}
%\left|\int_0^t{I_\epsilon\deltasr \normal\phi(\tau,0)(t-\tau)^{1/2}d\tau}\right|\leq \vol(\Omega)\|\deltasr \normal\phi\|_{L^\infty(U)}\int_0^t(t-\tau)^{1/2}d\tau=O(t^{3/2}),
%\end{equation}
%uniformly with respect to $\epsilon$. The third and last term involves $\partial_tI_\epsilon$, which can be handled with an integration by parts with respect to time. It's important to remark that this procedure makes sense thanks to Lemma \ref{lem:hp_idp_aux}. Thus, 
%\begin{align}
%\begin{split}
%\int_0^t{\partial_tI_\epsilon \normal\phi(\tau,0)(t-\tau)^{1/2}d\tau} &=I_\epsilon \normal\phi(\tau,0)(t-\tau)^{1/2}\Big|_{\tau=0}^{\tau=t}\\
																																%&\ \qquad\qquad\qquad\qquad+\frac{1}{2}\int_0^t{I_\epsilon \normal\phi(\tau,0)(t-\tau)^{-1/2}d\tau}
%\end{split}
%\\[1ex]
																															%&=-\int_{\omprime{\epsilon}}{\normal\phi \dvol}\sqrt{t}+\frac{1}{2}\int_0^t{I_\epsilon \normal\phi(\tau,0)(t-\tau)^{-1/2}d\tau}\\[1ex]
																															%&\xrightarrow{\epsilon\to 0}\frac{1}{2}\int_0^t{I \normal\phi(\tau,0)(t-\tau)^{-1/2}d\tau}.
%\end{align}
%\item[$(k=2)$] From \eqref{sum_iter_appl_L}, we know that $L^2\Lambda_\epsilon$ is of the form 
%\begin{equation}
%L^2\Lambda_\epsilon=\Lambda_\epsilon T_1+I_\epsilon T_2+\partial_t\Lambda_\epsilon T_3+\partial_tI_\epsilon T_4,
%\end{equation} 
%where $T_i\colon C_c^\infty(\neighbd)\to C_c^\infty(\neighbd)$ are operators in the sub-algebra of operators generated by $\{\deltasr,\normal\}$. Of course the first two terms are negligible, since, for $k=2$, $L^2\Lambda_\epsilon$ is coupled with $(t-\tau)^{3/2}$. The third term vanishes by Lemma \ref{lem:hp_idp_aux}: 
%\begin{equation}
%\int_0^t{\partial_t\Lambda_\epsilon T_3\phi(\tau,0)(t-\tau)^{3/2}d\tau}=0.
%\end{equation}
%Finally, the fourth term can be discussed as before, by integration by parts, therefore, denoting by $\varphi\coloneqq T_4\phi$,  we obtain
%\begin{align}
%\int_0^t{\partial_tI_\epsilon\varphi(\tau,0)(t-\tau)^{3/2}d\tau} &=I_\epsilon\varphi(\tau,0)(t-\tau)^{3/2}\Big|_{\tau=0}^{\tau=t}+\frac{3}{2}\int_0^t{I_\epsilon\varphi(\tau,0)(t-\tau)^{1/2}d\tau}\\[1ex]
																															%&=-\int_{\omprime{\epsilon}}{\varphi \dvol}\!\ t^{3/2}+\frac{3}{2}\int_0^t{I_\epsilon\varphi(\tau,0)(t-\tau)^{-1/2}d\tau}\\[1ex]
																															%&\xrightarrow{\epsilon\to 0}\frac{3}{2}\int_0^t{I\varphi(\tau,0)(t-\tau)^{1/2}d\tau}=O(t^{3/2}).
%\end{align}
%\end{mydescription}
%\hspace{\parindent}\textit{Step 4}: Write the asymptotic expansion for $I\phi(t,0)$.
%This last step is just a matter of gluing carefully all the previous steps together, starting from \eqref{lim_I_eps_after_duh}
%\begin{align}
%\begin{split}
%I\phi(t,0) &=-\frac{t^{3/2}}{2\sqrt{\pi}}\int_{\Omega}\normal^3\phi\dvol+\frac{2}{\sqrt{\pi}}\int_{\partial\Omega}{\phi(x)\dvol(x)}\sqrt{t}\\
					 %&\quad\qquad\qquad\qquad\qquad+\frac{1}{2\sqrt{\pi}}\int_0^t{I\normal\phi(\tau,0)(t-\tau)^{-1/2}d\tau}+O(t^{3/2})
%\end{split}
%\nonumber\\[1ex]
					 %&=\frac{2}{\sqrt{\pi}}\int_{\partial\Omega}{\phi(x)\dvol(x)}\sqrt{t}+\frac{1}{2\sqrt{\pi}}\int_0^t{I\normal\phi(\tau,0)(t-\tau)^{-1/2}d\tau}+O(t^{3/2}).\label{impl_2nd_order_exp_I_phi} 
%\end{align}
%As we would like to have explicit coefficients in the expansion of $I\phi$, \eqref{impl_2nd_order_exp_I_phi} doesn't fully satisfy us. To make it more precise, we use Theorem \ref{thm:1ord_Iphi}, which allows us to write
%\begin{align}
%\begin{split}
%\int_0^t{I\normal\phi(\tau,0)(t-\tau)^{-1/2}d\tau} &= \frac{2}{\sqrt{\pi}}\int_0^t{\int_{\partial\Omega}{\normal\phi \area}\tau^{1/2}(t-\tau)^{-1/2}d\tau}\\
																						 %&\quad\ \qquad\qquad\qquad+\int_0^tO(\tau)(t-\tau)^{-1/2}d\tau
%\end{split}\nonumber\\	
																						 %&= \sqrt{\pi}\int_{\partial\Omega}{\normal\phi \area}\!\ t+O(t^{3/2}),\label{very_diff_comp_integ}
%\end{align}
%since $\int_0^t{\tau^{1/2}(t-\tau)^{-1/2}d\tau}=t\frac{\pi}{2}$. Adding \eqref{very_diff_comp_integ} to what we had previously obtained in \eqref{impl_2nd_order_exp_I_phi}, we finally get statement \eqref{2nd_order_exp_I_phi}.
 %
%%Per questo integrale si fa prima la sostituzione $\frac{\tau}{t-\tau}=s^2$, si estrae un arcotangente, poi si fa la sostituzione $s=\tan u$ e si conclude.
%\end{proof}
%
%\begin{lem}
%\label{lem:uniform_est_reminder}
%Let $\phi\in C_c^\infty(\neighbd)$ and $\epsilon\in(0,\varepsilon)$. Then, the reminder 
%\begin{equation}
%\label{reminder_duh_m3}
%\int_0^t{\int_0^\infty{e(t-\tau,r,0)L^3I_\epsilon\phi(\tau,r)(t-\tau)^2dr}\ \negthinspace d\tau}
%\end{equation}
%is an $O(t^{3/2})$ as $t\to 0$, uniformly with respect to $\epsilon$.
%\end{lem}
%
%\begin{proof}
%We compute $L^3I_\epsilon$ using Lemma \ref{lem:iter_L}, which holds without any changes,
%\begin{align}
%L^3I_\epsilon &=\left(L\Lambda_\epsilon(-\normal^2+\deltasr)-LI_\epsilon\deltasr \normal+\partial_t(\Lambda_\epsilon \normal+I_\epsilon\deltasr)\normal\right)\normal+L(\Lambda_\epsilon \normal+I_\epsilon\deltasr)\deltasr\\
     %%&=\Bigg(\Big(\Lambda_\epsilon(-\normal^2+\deltasr)+\partial_tI_\epsilon-I_\epsilon\deltasr\Big)(-\normal^2+\deltasr)-(\Lambda_\epsilon \normal+I_\epsilon\deltasr)\deltasr\\
		%%&+\partial_t(\Lambda_\epsilon \normal+I_\epsilon\deltasr)\Bigg)\normal+\Bigg(\Big(\Lambda_\epsilon(-\normal^2+\deltasr)+\partial_tI_\epsilon-I_\epsilon\deltasr\Big) \normal+(\Lambda_\epsilon \normal+I_\epsilon\deltasr)\deltasr\Bigg)\deltasr\\
		 %&= I_\epsilon T_1+\Lambda_\epsilon T_2+\partial_tI_\epsilon T_3+\partial_t\Lambda_\epsilon T_4,
%\end{align}
%where $T_i\colon C_c^\infty(\neighbd)\to C_c^\infty(\neighbd)$ are operators in the sub-algebra of operators generated by $\{\deltasr,\normal\}$. Therefore, it's enough to estimate $I_\epsilon\phi,\Lambda_\epsilon\phi$ and their first time derivative, for suitably chosen functions $\phi\in C_c^\infty(\neighbd)$. Thus, rewriting \eqref{reminder_duh_m3} as a sum of four terms, we can estimate term by term. Since, we can estimate
%\begin{equation}
%|I_\epsilon\phi(t,r)|=|\int_{\om{r}}{(1-u_\epsilon(t,x))\phi(x)\dvol(x)}|\leq \int_{\om{r}}{|(1-u_\epsilon(t,x))\phi(x)|\dvol(x)}\leq\vol(\Omega)\|\phi\|_{L^\infty(U)}.
%\end{equation}
%uniformly with respect to the parameter $\epsilon$, the first one gives
%\begin{equation}
%\left|\int_0^t{\int_0^\infty{e(t-\tau,r,0)I_\epsilon\phi(\tau,r)(t-\tau)^2dr}\ \negthinspace d\tau}\right|\leq \hat{C}_1(\phi,\Omega)\int_0^t{(t-\tau)^2dr\ \negthinspace d\tau}=C_1(\phi,\Omega)t^3,
%\end{equation}
%recalling that $\int_0^\infty{e(t-\tau,r,0)dr}=O(1)$. To estimate the second one, we make use of the co-area formula, precisely 
%\begin{align}
%\begin{split}
%\Bigg|\int_0^t\int_0^\infty e(t-\tau,r,0)&\Lambda_\epsilon\phi(\tau,r)(t-\tau)^2dr\ \negthinspace d\tau\Bigg| \\
																%&= \Bigg|\int_0^t\int_0^\infty e(t-\tau,r,0)\int_{\bdom{r}}{(1-u_\epsilon(t,y))\phi(y)d^{n-1}(y)}(t-\tau)^2dr\ \negthinspace d\tau\Bigg|
%\end{split}
%\\[1ex]
																																																								 %&=\left|\int_0^t{\int_{\Omega}{e(t-\tau,\delta(x),0)(1-u_\epsilon(t,x))\phi(x)\dvol(x)}(t-\tau)^2\ \negthinspace d\tau}\right|\\[1ex]
																																																								 %&\leq \frac{\vol(\Omega)}{\sqrt{\pi}}\|\phi\|_{L^\infty(U)}\int_0^t{(t-\tau)^{3/2}\ \negthinspace d\tau}=C_2(\phi,\Omega)t^{5/2},
%\end{align}
%and again this estimate is uniform with respect to $\epsilon$. To conclude, it suffices to provide a uniform estimate for $\partial_tI_\epsilon$, being the case with $\partial_t\Lambda_\epsilon$ essentially equal. To deal with this term is enough to perform an integration by parts with respect to the time variable, obtaining
%\begin{align}
%\begin{split}
%\Bigg| \int_0^t\int_0^\infty e(t-\tau,r,0)&\partial_tI_\epsilon\phi(\tau,r)(t-\tau)^2dr\ \negthinspace d\tau \Bigg| \\
																%&\leq \hat{C}_3(\phi,\Omega)t^2+\hat{C}_1(\phi,\Omega) \int_0^\infty\int_0^t \left|\partial_t\left(e(t-\tau,r,0)(t-\tau)^2\right)\right|d\tau \ \negthinspace dr
%\end{split}
%\\[1ex]
																																																								 %&\leq C_3(\phi,\Omega)t^{3/2},
%\end{align}
%having used Lemma \ref{lem:hp_idp_aux} to evaluate
%\begin{align}
%\Bigg|\int_0^\infty e(t-\tau,r,0)I_\epsilon\phi(\tau,r)(t-\tau)^2dr\Big|_{\tau=0}^{\tau=t}\Bigg| &= \left|\int_0^\infty e(t,r,0)I_\epsilon\phi(0,r)dr\right| t^2\\[1ex]
																																													 %&= \left|\int_{\omprime{\epsilon}} \phi(x)\left(\smallerint{0}{\delta(x)}{e(t,r,0)dr}\right)\dvol(x)\right| t^2\\[1ex]
																																													 %&\leq \vol(\Omega)\|\phi\|_{L^\infty(U)}t^2=\hat{C}_3(\phi,\Omega)t^2.
%\end{align}
%\end{proof}

%In this section, we develop the machinery to achieve a full asymptotic expansion, as $t\to 0$, of the function $I\phi(t,0)$, via an approximation technique. We have already showed that a first order asymptotic expansion exists, applying the Duhamel's principle. 

The iterations of the Duhamel's principle lead to the definition of the following family of operators acting on the space of functions $C_c^\infty(\neighbd)$, which lies in the algebra $\A\coloneqq\spn\{\deltasr,\normal\}$, where $\normal$ is defined as in \eqref{eqn:sr_normal}:
\begin{equation}
\label{eqn:1st_fam}
\begin{cases}
R_{kj}=-(\normal^2-\deltasr)R_{k-1,j}+\normal S_{k-1,j}\\
S_{kj}=\normal R_{k-1,j-1}-\deltasr\normal R_{k-1,j}+\deltasr S_{k-1,j}
\end{cases}
\qquad\forall\,k\geq 1,\,j\geq 0,
\end{equation}
having set $R_{00}=Id$, $S_{00}=0$ and $R_{kj}=S_{kj}=0$ whenever $k$ or $j$ is a negative integer. Moreover, define:
\begin{equation}
\label{eqn:def_Zalpha}
Z_k\coloneqq\sum_{j=0}^{k-1}\{k,j-1\}R_{k+j-1,j}\qquad\text{and}\qquad\alpha_k\coloneqq\sum_{j=0}^{k+1}\{k,j\}S_{k+j,j},
\end{equation}
having set: 
\begin{equation}
\{k,j\}\coloneqq \frac{\Gamma(k+j+1/2)}{(k+j)!\Gamma(k+1/2)},
\end{equation}
and $\Gamma$ denotes the usual Gamma function. Finally, let $D_k$ be the operators in $\A$, defined inductively by the formulas:
\begin{equation}
\label{eqn:recurs_op}
\begin{split}
&D_1 =\frac{2}{\sqrt{\pi}}Id,\\
&D_{2n} =\frac{1}{\sqrt{\pi}}\sum_{i=1}^n\frac{\Gamma(i+1/2)\Gamma(n-i+1/2)}{n!}D_{2i-1}\alpha_{n-i},\\
&D_{2n+1} =\frac{1}{\sqrt{\pi}}Z_{n+1}+\frac{1}{\sqrt{\pi}}\sum_{i=1}^n\frac{i!\Gamma(n-i+1/2)}{\Gamma(n+3/2)}D_{2i}\alpha_{n-i}.
\end{split}
\end{equation}
Having defined these operators, we are able to give a recursive formula which explicitly computes the coefficients of the small-time asymptotic expansion of the function $I\phi(t,0)$. We state here the main result and we refer to Appendix \ref{app:B} for a complete proof, since the Riemannian's one extends without any changes to the \sr case.\todo{Se si vuole togliere l'appendice B, qui si può mettere una referenza} 

\begin{thm}
\label{thm:asymp_Iphi} Under the same hypotheses of Lemma \ref{lem:op_LI}, let $\phi\in C_c^\infty(\neighbd)$. Then, for any $m\in\N$:
\begin{equation}
\label{eqn:asymp_Iphi}
I\phi(t,0)=\sum_{k=1}^m\beta_k(\phi)t^{k/2}+O(t^{(m+1)/2}),\qquad\text{as }t\to 0,
\end{equation}
where the $k$-th coefficient is $\beta_k(\phi)\coloneqq\int_{\partial\Omega}D_k\phi$.
\end{thm}

\subsection{Heat content asymptotic expansion}

\begin{thm}
\label{thm:full_asymp}
Let $M$ be a \sr manifold with volume $\omega$ and $\Omega\subset M$ be a connected and relatively compact subset of $M$, whose boundary is a smooth hypersurface with no characteristic points. Denote by $\delta\colon\bar\Omega\to[0,\infty)$ be the distance function from $\partial\Omega$. Consider the Dirichlet problem for the heat equation \eqref{eqn:dir_prob} on $\Omega$. Then, denoting with $Q(t)$ the \sr heat content associated with $\Omega$, $Q(t)$ has a full asymptotic expansion as $t\to 0$. In particular, 
\begin{equation}
\label{eqn:full_asymp}
Q(t)\sim\sum_{k=0}^{\infty}a_kt^{k/2},\qquad\text{as }t\to 0,
\end{equation}
where $a_0\coloneqq\vol(\Omega)$ and $a_k\coloneqq-\beta_k(1)=-\int_{\partial\Omega}D_k(1)$.
\end{thm}

\begin{rmk}
The operators \eqref{eqn:recurs_op} were defined on the set of functions supported near the boundary, namely $C_c^\infty(\neighbd)$, where $\neighbd\coloneqq\{x\in\bar\Omega;\delta(x)<\smallpar\}$, nevertheless, the coefficients $a_k$ are well-defined, since it makes sense to evaluate $D_k$'s on the function in $C_c^\infty(\neighbd)$, which is definitely $1$ near the boundary and, then compute its integral on it.
\end{rmk}

\begin{proof}
Recall the definition of the function $I\phi$, for $\phi\in C_c^\infty(\neighbd)$:
\begin{equation}
I\phi(t,r)=\int_{\om{r}}\left(1-u(t,x)\right)\phi(x)\dvol(x),\qquad (t,r)\in (0,\infty)\times [0,\infty).
\end{equation} 
Hence, it is clear that, if we choose $\phi=1$, when evaluated at $r=0$,
\begin{equation}
\label{eqn:I1_heat}
I[1](t,0)=\vol(\Omega)-Q(t).
\end{equation}
Therefore, we would like to apply Theorem \ref{thm:asymp_Iphi} to the function $I[1](t,0)$, however $1\notin C_c^\infty(\neighbd)$, since it is not $0$ in $\om{\smallpar}$. To avoid this difficulty, we can employ the \sr principle of not feeling the boundary: let $\eta$ be a bump function compactly supported in $U_{\smallpar/2}^c$\footnote{the complement is assumed to be in $\bar{\Omega}$, namely $U_{\smallpar/2}^c=\bar\Omega\setminus U_{\smallpar/2}$} and equal to $1$ in $\bar{\om{\smallpar}}$. Writing $1=(1-\eta)+\eta$, we see that now $1-\eta\in C_c^\infty(\neighbd)$, therefore we may apply Theorem \ref{thm:asymp_Iphi} to $I[1-\eta](t,0)$, obtaining, for any $m\in\N$:
\begin{equation}
I[1-\eta](t,0)=\sum_{k=1}^m\beta_k(1-\eta)t^{k/2}+O(t^{(m+1)/2}),\qquad\text{as }t\to 0.
\end{equation}
On the other hand, $\supp(\eta)$ is bounded away from $\partial\Omega$, thus, applying Theorem \ref{thm:not_feel_bd}, for any $m\in\N$, we have:
\begin{equation}
I\eta(t,0)=O(t^m),\qquad\text{as }t\to 0.
\end{equation}
Adding up these facts, we get that, for any $m\in\N$: 
\begin{equation}
\label{eqn:inter_comp}
I[1](t,0)=I[1-\eta](t,0)+I\eta(t,0)=\sum_{k=1}^m\beta_k(1-\eta)t^{k/2}+O(t^{(m+1)/2}),
\end{equation}
as $t\to 0$. But the coefficients of the expansion, appearing in the right-hand side of \eqref{eqn:inter_comp}, are integrals computed over $\partial\Omega$, where the function $1-\eta$ is definitely $1$, being $\eta$ supported on $U_{\varepsilon/2}^c$, hence:
\begin{equation}
\beta_k(1-\eta)=\int_{\partial\Omega}D_k(1-\eta)=\int_{\partial\Omega}D_k(1)=\beta_k(1),\qquad\forall\,k\in\N.
\end{equation}
This concludes the proof since, by formula \eqref{eqn:I1_heat}, we may write, for any $m\in\N$: 
\begin{equation}
Q(t)=\vol(\Omega)-I[1](t,0)=\vol(\Omega)-\sum_{k=1}^m\beta_k(1)t^{k/2}+O(t^{(m+1)/2}),\qquad\text{as }t\to 0.
\end{equation}
\end{proof}

\todo{Inserire esempio di $\hei$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SEMBRA CHE NEL LAVORO DI TYSON IL SECONDO COEFFICIENTE ABBIA SEGNO + E NON -. BISOGNA CONTROLLARE TUTTI I SEGNI
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






==> convergence.tex <==
\section{Convergence of the heat semi-group of the Riemannian variation}\label{app:A}
%We recall some general facts about sequences of unbounded operator and heat semi-groups and we prove some technical results needed in the proof of Theorem \ref{thm:not_feel_bd}.
%
%\begin{defn}
%Let $A_\eps$, $A$ be self-adjoint (possibly unbounded) operators on $\hil$, for any $\eps\in\R$. Then, the 1-parameter family $\{A_\eps\}_{\eps\in\R}$ is said to converge to $A$ in the \emph{strong resolvent sense} if $R_\lambda(A_\eps)\to R_\lambda(A)$, as $\eps\to 0$, strongly for all $\lambda$ with $\im(\lambda)\neq 0$, i.e.
%\begin{equation}
%R_\lambda(A_\eps)\varphi\xrightarrow{\eps\to 0} R_\lambda(A)\varphi, \qquad\forall\, \varphi\in \hil,
%\end{equation}
%where $R_\lambda(A)=(\lambda-A)^{-1}$ is the resolvent operator of $A$ associated with $\lambda$. 
%\end{defn}
%
%For a self-adjoint operator $A$ on $\hil$, such that its spectrum $\spec{A}$ is bounded above, we can define by the spectral theorem, for $t\geq 0$, the one-parameter strongly continuous semi-group of operators $e^{tA}:\hil\to \hil$.
%
%\begin{thm}
%\label{thm:trotter}
%Let $A_\eps$, $A$ be self-adjoint (possibly unbounded) operators on $\hil$, for any $\eps\in\R$, and assume that their spectra are uniformly bounded, i.e. there exists $\gamma\in\R$ such that $\lambda\leq \gamma$, $\forall\, \lambda\in\spec{A} \cup\spec{A_\eps}$. If $A_\eps\to A$, as $\eps\to 0$ in the strong resolvent sense, then $e^{tA_\eps}\to e^{tA}$, as $\eps\to 0$, strongly for any $t\geq 0$. 
%Moreover, for any $T>0$:
%\begin{equation}
%\label{eqn:key_rel}
%e^{tA_\eps}\varphi\xrightarrow{\eps\to 0} e^{tA}\varphi,\qquad \forall\, \varphi\in \hil, \text{ uniformly on } [0,T].
%\end{equation}
%\end{thm}
%
%\begin{proof}
%By the Stone-Weierstrass Theorem, the set of polynomials in $(x+i)^{-1}$ and $(x-i)^{-1}$ is dense in the set of continuous function vanishing at infinity, denoted by $C_{\infty}(\R)$. Thus, for $f\in C_{\infty}(\R)$, and $\delta>0$, we can find a polynomial $p\in\R[s,t]$, such that
%\[
%\|f(x)-p((x+i)^{-1},(x-i)^{-1})\|_{L^\infty(\R)}\leq \delta/3.
%\]
%Therefore, using the spectral theorem \cite[Thm.\ VIII.5]{MR0493419}, we get:
%\begin{equation}
%\|f(A)-p((A+i)^{-1},(A-i)^{-1})\|_{\B(\hil)}\leq \delta/3,
%\end{equation}
%and also
%\begin{equation}
%\|f(A_\eps)-p((A_\eps+i)^{-1},(A_\eps-i)^{-1})\|_{\B(\hil)}\leq \delta/3.
%\end{equation}
%On the other hand, if $A_\eps\to A$ in the strong resolvent sense, then
%\begin{equation}
%p((A_\eps+i)^{-1},(A_\eps-i)^{-1})\xrightarrow{\eps\to 0} p((A+i)^{-1},(A-i)^{-1}),
%\end{equation}
%strongly in $\hil$. Therefore, it follows that
%\begin{equation}
%\label{eqn:conv_C_infty}
%f(A_\eps)\varphi\xrightarrow{\eps\to 0} f(A)\varphi, \qquad \forall\,\varphi\in \hil, \ \forall\,f\in C_{\infty}(\R).
%\end{equation}
%We would like to apply \eqref{eqn:conv_C_infty} to the function $h(x)= e^{tx}$, to obtain the strongly convergence of semi-groups, however $h$ does not belong to $C_\infty(\R)$. To avoid this difficulty, define the functions $g_m(x)= e^{-x^2/m}$, for any $m>0$. These functions lie in $C_{\infty}(\R)$ and, in addition, $hg_m\in C_{\infty}(\R)$. Hence, from \eqref{eqn:conv_C_infty}, we obtain, for any $\varphi\in \hil$ and $m>0$
%\begin{align}
%\|g_m(A_\eps)\varphi-g_m(A)\varphi\|_\hil&\xrightarrow{\eps\to 0}0,\\
%\|h(A_\eps)g_m(A_\eps)\varphi-h(A)g_m(A)\varphi\|_\hil&\xrightarrow{\eps\to 0}0.
%\end{align}
%On the other hand, $g_m(x)\nearrow 1$ pointwise as $m\to+\infty$, hence, employing again the spectral theorem, $g_m(A)\to Id$, in $\B(\hil)$, as $m\to+\infty$. Therefore, choosing $m$ sufficiently big, $\eps$ sufficiently small, we have:
%\begin{equation}
%\|g_m(A_\eps)\varphi-\varphi\|_\hil\leq \|g_m(A_\eps)\varphi-g_m(A)\varphi\|_\hil+\|g_m(A)\varphi-\varphi\|_\hil\leq\eps.
%\end{equation}
%Finally, for suitable choices of $m$ and $\eps$, we obtain:
%\begin{align}
%\|h(A_\eps)\varphi-h(A)\varphi\|_\hil & \leq\begin{aligned}[t] &\|h(A_\eps)g_m(A_\eps)\varphi-h(A)g_m(A)\varphi\|_\hil \\
																																		 %&+\|h(A_\eps)\|_{\B(\hil)}\|g_m(A_\eps)\varphi-\varphi\|_\hil \\
																																		%&+\|h(A)\|_{\B(\hil)}\|g_m(A)\varphi-\varphi\|_\hil\end{aligned}\\
														 %&\leq \delta+e^{\gamma t}\delta+e^{\gamma t}\delta,
%\end{align}
%where in the last inequality, we have used the uniform bound on the spectra of the operators $A_\eps,A$. This concludes the proof.
%\end{proof}
%
%We now recall one sufficient condition for convergence in the strong resolvent sense.
%
%\begin{defn}
%Assume that $A$ is a closed (possibly unbounded) operator on $\hil$. A linear dense subset $D\subset\dom(A)$ is called a \emph{core} for $A$ if $\overline{A|_{D}}=A$.
%\end{defn}
%
%\begin{thm}
%\label{thm:crit_StReCo}
%Let $A_\eps$, $A$ be self-adjoint (possibly unbounded) operators on $\hil$, for any $\eps\in\R$. Assume that $D$ is a common core for all $A_\eps$, $A$. If $A_\eps\varphi\to A\varphi$ in $\hil$, as $\eps\to 0$, for each $\varphi\in D$, then $A_\eps\to A$ in the strong resolvent sense, as $\eps\to 0$.
%\end{thm}
%\begin{proof}
%See \cite[Thm.\ VIII.25]{MR0493419}.
%\end{proof}

We prove some technical results needed in the proof of Theorem \ref{thm:not_feel_bd}. Here, $\hil$ denotes a Hilbert space and any unbounded linear operator defined on $\hil$ is tacitly assumed to be densely defined. 

\begin{defn}
Assume that $A$ is a closed (possibly unbounded) operator on $\hil$. A linear dense subset $D\subset\dom(A)$ is called a \emph{core} for $A$ if $\overline{A|_{D}}=A$.
\end{defn}

\begin{thm}[Trotter-Kato]
\label{thm:trotter}
Let $A_\eps$, $A$ be self-adjoint (possibly unbounded) operators on $\hil$, for any $\eps\in\R$, such that their spectra are uniformly bounded, i.e. there exists $\gamma\in\R$ such that $\lambda\leq \gamma$, $\forall\, \lambda\in\spec{A} \cup\spec{A_\eps}$. Assume that $D$ is a core for $A$, such that the following properties hold:
\begin{enumerate}[label=\roman*)]
\item $D\subset\dom(A_\eps)$,
\item $A_\eps\varphi\to A\varphi$ in $\hil$, as $\eps\to 0$, for each $\varphi\in D$.
\end{enumerate}
Then $e^{tA_\eps}\to e^{tA}$, as $\eps\to 0$, strongly for any $t\geq 0$. 
Moreover, for any $T>0$:
\begin{equation}
\label{eqn:key_rel}
e^{tA_\eps}\varphi\xrightarrow{\eps\to 0} e^{tA}\varphi,\qquad \forall\, \varphi\in \hil, \text{ uniformly on } [0,T].
\end{equation}
\end{thm}

\begin{proof}
.\todo{Inserire referenza}
\end{proof}

\begin{cor}
\label{cor:conv_appr}
Let $(\D,g)$ be a \sr structure on $M$ and $\{(M,g_\eps)\}_{\eps \in \R}$ be a Riemannian variation. Fix a smooth volume $\omega$ on $M$ and let $\Omega\subseteq M$ be an open, relatively compact set. Let $\Delta_\eps$, $\deltasr$ be the weighted Dirichlet $\eps$-Riemannian and \sr Laplacian respectively. Then, for any $T>0$
\begin{equation}
\label{eqn:conv_sol}
e^{t\Delta_\eps}\varphi\xrightarrow{\eps\to 0} e^{t\deltasr}\varphi,\qquad \forall\, \varphi\in L^2(\Omega), \text{ uniformly on } [0,T].
\end{equation}
\end{cor}

\begin{proof}
Set here $\hil=L^2(\Omega,\omega)$, while $A_\eps=\Delta_\eps$, for any $\eps\in\R$ and $A=\deltasr$ are the Dirichlet Laplacians of $(M,g_\eps)$ and the sub-Laplacian, i.e.\ the Friedrichs extensions of the Dirichlet energy functionals, defined respectively by:
\begin{equation}
\mathcal{E}_\eps(f)=\int_\Omega2H_\eps(df)\dvol,\qquad \mathcal{E}(f)=\int_\Omega2H(df)\dvol,\qquad\forall f\in C_c^\infty(\Omega),
\end{equation}
where $H_\eps,H$ are respectively the $\eps$-Riemannian and the \sr Hamiltonian. It is enough to check that these operators satisfy the hypotheses of Theorem \ref{thm:trotter}. First of all, both $A$ and $A_\eps$ have negative spectrum, so that their spectra is uniformly bounded by $0$. Second of all, a core for $A$ is the set
\begin{equation}
D=\{ f\in C^\infty(\bar\Omega) \mid f|_{\partial\Omega} = 0\}.
\end{equation}
This is a well-known fact in the Euclidean case, but the proof (e.g.\ see \cite[Prop.\ 1, p.\ 264]{MR0493421}) holds unchanged in the (sub-)Riemannian case, by the spectral theorem. Thus, $D\subset\dom(A_\eps)$, for any $\eps>0$.

Using the explicit expressions of $\Delta$ and $\Delta_\eps$ on smooth functions, in terms of a generating frame for the Riemannian variation \eqref{eqn:approx_lapl}, we get that:
\begin{equation}
A_\eps\varphi\xrightarrow{\eps\to 0}A\varphi,\qquad\forall\,\varphi\in D,
\end{equation}
uniformly on $\Omega$, and hence also on $\hil$. Consequently, applying Theorem \ref{thm:trotter}, we obtain the convergence \eqref{eqn:conv_sol}.
\end{proof}

We prove now Lemma \ref{lem:improved_conv}. We recall here its statement for the reader's convenience. 

\begin{lem*}
Let $M$ be a sub-Riemannian manifold, equipped with a smooth measure $\omega$, and let $\Omega \subset M$ be an  open relatively compact subset with smooth boundary. Fix $\{(M,g_\eps)\}_{\eps\in\R}$, a Riemannian variation of $M$. Let $\eta\in C^{\infty}_c(\Omega)$, with support separated from $\partial\Omega$. Then, for any $T>0$ and any integer $k\geq 1$, we have:

\begin{equation}
\label{eqn:improved_conv2} 
\partial_t^ke^{t\Delta_\eps}\eta\xrightarrow[\|\cdot\|_{L^2}]{\eps\to 0}\partial_t^ke^{t\deltasr}\eta,\qquad\text{uniformly w.r.t. }t\in (0,T).
\end{equation}
\end{lem*}

\begin{proof}
First of all, let $\{\psi_\eps\}_{\eps> 0}\subset L^2(\Omega)$ be a convergent sequence to $\psi\in L^2(\Omega)$, then, for any $\rho>0$, choosing $\eps$ suitably small, we have: 
\begin{align}
\|e^{t\Delta_\eps}\psi_\eps-e^{t\deltasr}\psi\|_{L^2} &\leq \|e^{t\Delta_\eps}\psi_\eps-e^{t\Delta_\eps}\psi\|_{L^2}+\|e^{t\Delta_\eps}\psi-e^{t\deltasr}\psi\|_{L^2}\nonumber\\
																									 &\leq \|e^{t\Delta_\eps}\|_{\B(L^2)}\|\psi_\eps-\psi\|_{L^2}+\|e^{t\Delta_\eps}\psi-e^{t\deltasr}\psi\|_{L^2}\nonumber\\
																									 &\leq \|\psi_\eps-\psi\|_{L^2}+\|e^{t\Delta_\eps}\psi-e^{t\deltasr}\psi\|_{L^2}\leq \rho, \label{est:improved_conv}
\end{align}
where, in the last inequality, we have used the fact the heat semi-group is a contraction semi-group for any $\eps$, therefore its operator norm is smaller than $1$, and Corollary \ref{cor:conv_appr}. We remark that, since the estimate \eqref{est:improved_conv} is uniform with respect to the time variable, also the convergence remains uniform on $[0,T]$. 

Let now $\eta\in C_c^{\infty}(\Omega)$ be as in the statement. Since $\eta$ is supported away from $\partial \Omega$, $\Delta^k_\eps\eta \in C^\infty_c(\Omega) \subset \dom(\Delta_\eps)$ for all $k\geq 1$ and $\eps \in \R$. Since on $\dom(\Delta_\eps)$ the heat-semigroup commutes with $\Delta_\eps$, it holds: 
\begin{equation}
\partial_t^ke^{t\Delta_\eps}\eta = \partial_t^{k-1}\Delta_\eps e^{t\Delta_\eps}\eta=\partial_t^{k-1}e^{t\Delta_\eps}\Delta_\eps\eta
																 = \dots =  e^{t\Delta_\eps}\Delta_\eps^k\eta=e^{t\Delta_\eps}\eta_\eps, \qquad \forall\, t>0,
\end{equation}
where we defined $\eta_\eps=\Delta_\eps^k\eta \in C^\infty_c(\Omega)$.

It follows directly from the expression \eqref{eqn:approx_lapl} that:
\begin{equation}
\eta_\eps=\Delta_\eps^k\eta\xrightarrow{\eps\to 0}\deltasr^k\eta,
\end{equation}
uniformly on $\Omega$, and in particular also in $L^2(\Omega$). Therefore, using \eqref{est:improved_conv}:
\begin{equation}
e^{t\Delta_\eps}\eta_\eps\xrightarrow[\|\cdot\|_{L^2}]{\eps\to 0} e^{t\deltasr}\deltasr^k\eta=\partial_t^ke^{t\deltasr}\eta, \qquad \text{uniformly w.r.t. }t\in(0,T),
\end{equation}
concluding the proof.
\end{proof}




